Wikipedia and Westminster: Quality and Dynamics of Wikipedia Pages about UK Politicians

Wikipedia is a major source of information providing a large variety of content online, trusted by readers from around the world. Readers go to Wikipedia to get reliable information about different subjects, one of the most popular being living people, and especially politicians. While a lot is known about the general usage and information consumption on Wikipedia, less is known about the life-cycle and quality of Wikipedia articles in the context of politics. The aim of this study is to quantify and qualify content production and consumption for articles about politicians, with a specific focus on UK Members of Parliament (MPs). First, we analyze spatio-temporal patterns of readers' and editors' engagement with MPs' Wikipedia pages, finding huge peaks of attention during election times, related to signs of engagement on other social media (e.g. Twitter). Second, we quantify editors' polarisation and find that most editors specialize in a specific party and choose specific news outlets as references. Finally we observe that the average citation quality is pretty high, with statements on 'Early life and career' missing citations most often (18%).

==> HT Arxiv/sections/background.tex <==

\section{Background and Related Work}

We now provide some brief background on the UK political system and then discuss related research work on different themes.

\textbf{The UK House of Commons.} The UK Parliament has two chambers, of which the House of Commons is the lower chamber. It comprises 650 Members of Parliament (MPs) who are elected to represent constituencies by the First-Past-The-Post (FPTP) system. Due to the operation of FPTP, most MPs belong to one of two main parties, Conservative and Labour.
% which are on the centre-right and centre-left of the political spectrum respectively.
The UK Parliament created its first website in 1996, featuring a range of parliamentary papers, including Hansard~\cite{hansard}, the near-verbatim report of proceedings of both houses. %From the early 2000s the parliament has placed an increasing emphasis on improving public understanding and knowledge of its work~\cite{ukadmin,ukmodern}. 
The parliament website now has extensive information about individual MPs and how parliament works~\cite{ukmembers}.

%\miriam{start generally with works ; works measuring engagement with editors; finally, focus on politics studies. And at the end, explain why this work is different from everything you have mentioned.}\pushkal{Updated}



\textbf{Editors' Engagement with Wikipedia}
%Editors are the backbone of the Wikipedia platform. 
Wikipedia is a platform where thousands of volunteers revise and add content constantly~\cite{iba2010analyzing}.  The work which is most closely relevant to ours is a recent study which looked at Wikipedia pages of members of Germany's parliament (Bundestag)~\cite{gobel2018political, reif2017politicians}. They show that German MPs use Wikipedia pages to enhance their image. Changes in pages are made at regular intervals, and significant peaks in the number of edits are associated with pursuing re-election. In ~\cite{gobel2018political}, authors use IP based public user edits to identify edits made from within the Bundestag and characterise types of changes. %Also, Local (non so popular) articles are less focused by the editors~\cite{graham2015digital}. .

%\pushkal{Edward suggested to delete this paragraph:
%\textbf{Online Political communication.}
%With the rise in internet, political communication via online platforms is also increasing. Early studies in this field include UK MPs use of social media such as Twitter\cite{jackson2011microblogging,graham2013between,leston2013deeply} which they use  to impress and serve their constituents. %Parliaments across the world use social media more to report parliamentary business than for interacting with citizens~\cite{leston2013deeply}. Later study finds that 
%Studies showed that there is a ten folds increase from 2011 to 2017 on MPs using Twitter, and that MPs collectively have 13 Millions followers ~\cite{agarwal2019tweeting}. MPs want to engage online and selectively reply to constituents, to positive tweets and to people they follow ~\cite{agarwal2019tweeting}. The increased usage has also raised concerns about the amount of abusive tweets MPs get on these platforms ~\cite{gorrell2018twits,mertens2019tweet}. According to these studies, party and gender lines play a dominant role in the type and cases of online abuse.}

%After understanding these extends of studies we presents engagement with Wikipedia of UK MPs. 


\textbf{Wikipedia pages quality.}
There are several works on various dimensions of page quality. Certain editors proclaim their political leaning and form communities~\cite{neff2013jointly}. Polarised teams--those consisting of a balanced set of politically diverse editors--may create articles of higher quality than politically homogeneous teams~\cite{shi2019wisdom}. 
Citations play a major role in the monitoring of information quality on Wikipedia. To help with this, the \emph{Citation Need} classifier by ~\cite{Redi:2019:CNT:3308558.3313618} determines if a statement requires a citation.

%and providing quality and topic labels.

To the best of our knowledge, this is the first study looking at political communication in Wikipedia in the context of UK Members of Parliament. %Also given the recent events of ups and downs in the UK since 2016 Brexit referendum the dataset also becomes large and novel. 
While ~\cite{gobel2018political} focuses on edits coming from inside the German Parliament, our study focuses on a much larger group of edits, and for the first time studies partisanship and neutrality of the Wikipedia editors of the MP wiki pages. 

==> HT Arxiv/sections/dataset.tex <==
\section{Dataset}\label{sec:dataset}
Following are details of our dataset of Wikipedia articles for the 650 MPs elected in the 2017 general election. 
We summarise the distribution of the dataset in Figure~\ref{fig:stats}.


\textbf{Page Views} 
To understand readers' engagement, we collect the daily page views data on all articles, using Wikimedia's~\footnote{The Wikimedia foundation host projects and websites such as Wikipedia.} page view API.\footnote{\url{https://tools.wmflabs.org/pageviews/}, Accessed 26 Feb 2020} 
%For making calls to the API we make use of an R library `pageviews'\footnote{cran.r-project.org/web/packages/pageviews/pageviews.pdf} which provides functions for calling the API and storing responses in a data frame. 
We use the earliest possible day that can be set (i.e. 01 July 2015) in the Wiki API query, and obtain daily page views per MP page until 30 June 2019.  In total, we observe over 160M views for 650 pages during this period. 

\textbf{Page Edits} 
%Using list of 650 MPs 
We crawl the history of page edits for all 650 MPs from 01 June 2002 to 28 Aug 2019. We store in total 231k edits. These edits are made by 43k unique editors.
Across all edits we see that 55k edits are made using public IP addresses, which is shown as the username for anonymous editors. 

\textbf{Page Content}
To understand the content of the pages, we also collect page text as HTML dumps as on 18 July 2019. %In total, we dump paragraphs having 683k words.
From these dumps, we extract the paragraph text, section titles, the citations list and other metadata for each page. %We find that some MPs such as \emph{David Duguid} \footnote{\url{en.wikipedia.org/wiki/David\_Duguid\_(politician)}, Accessed on 18 July 2019} have just few lines in pages.

\textbf{MPs Information} 
We obtain additional profile information of MPs using Wikidata.org, a free Wikimedia foundation knowledge base.
Wikidata provides information about MPs' gender, party, year of page creation and position held in the Parliament. 
We identify the role of each MP in politics, which is Wikidata's \emph{Position held (P39)} property.
%\footnote{\url{wikidata.org/wiki/Property:P39}, Accessed on 26 Feb 2020}. % and obtain 2343 positions of MPs so far
For example, for the current prime minister \emph{Boris Johnson} his positions held include: \emph{Mayor of London, Secretary of State, Member of Parliament, Prime Minister and Leader of the Conservative Party}.
%\footnote{\url{wikidata.org/wiki/Q180589}, Accessed on 26 Feb 2020} 
%\footnote{  \url{en.wikipedia.org/wiki/Kenneth\_Clarke}, Accessed 09 Feb 2020}

\textbf{Additional Data}
We obtain additional baseline data from Wikipedia and Twitter. We collect MPs' interactions on Twitter, such as number and popularity of mentions across 2 months from~\cite{agarwal2019tweeting}. For Wikipedia, we crawl page views for \emph{Sportspeople} (footballers) and \emph{actors}. These categories are popular biographies of living people in the UK\footnote{\url{www.wikidata.org/wiki/Wikidata:Living_people/uk},  Accessed 15 Feb 2020}. We randomly sample 1000 pages from a Wikidata page list of these two categories.



\begin{figure*}[htb]
    \centering
    % \subfloat[Page creations] {
    %     \includegraphics[width=0.33\textwidth]{figures/postisionAndCreation.png}
    %     \label{fig:pageYear}
    % }
    %     \begin{figure}
    % \centering
    \subfloat[Dataset Counts]{
      \includegraphics[width=0.3\textwidth]{figures/basicStats.pdf}
      \label{fig:stats}
      %\vspace{-1cm}
    % \end{figure}
    }
    \subfloat[Page Views] {
        \includegraphics[width=.31\textwidth]{figures/viewsMPActPlay.png}
        \label{fig:views}
    }
    \subfloat[Constituency Edits] {
        \includegraphics[width=.3\textwidth]{figures/constiCDFMap.png}
        \label{fig:map}
    }
    \caption{Spatio-temporal patterns. %(a) Page creation and first position held as an MP.
    (a) CDF (Cumulative Distribution Function) of number of views, edits and editors per MP.
    (b) Page views of MPs pages and baselines (footballers and  actors in the UK). 
    (c) CDF of constituency engagement. Inset: All edits from constituencies of Greater London.}
    %\vspace{-0.5cm}
\end{figure*}
    



==> HT Arxiv/sections/discussion.tex <==
\section{Discussion}\label{sec:discussion}
In this paper, we discussed important dynamics of attention and content production in the context of Wikipedia articles focusing on UK Members of Parliament. We find evidence of specialization in contribution patterns of the editors of MP pages. %, and signals of  readers' satisfaction in terms of information need. 
With our analysis, we contribute to the broader field of online political communication studies, and shed light on behavior of contributors to the largest online encyclopedia.
% The paper discusses important aspects of spatio-temporal patterns, polarisation and quality of UK MPs' Wikipedia pages. Given the importance of these pages within the matrix of 21st Century political communications, our study contributes to understanding the underlying patterns of editing and identifying gaps. 
We summarise our findings as follows:

\textbf{Spatio-Temporal Peaks of Engagement.} Similar to previous work, we find that MP page creations, views and edits are strongly aligned with media coverage and election periods. Furthermore, we find that only a small fraction of edits come from within the constituency of the MP, whereas the majority of anonymous edits come from Central London where the political centre of the UK lies. Collectively, these findings suggest that attention peaks are localized both in time and space, thus introducing potential vulnerabilities to the integrity of the content. Researchers working on monitoring and detecting coordinated disinformation attacks in political communications might benefit from these findings and further investigate how these peaks of attention might affect temporarily the quality of content on Wikipedia MP pages. 

\textbf{Polarisation Dynamics.}  We observe signals of partisanship among edits and domains of citations on papers. Many editors  contribute to the pages of MPs of one party, and we also see communities of editors who collectively focus on each party. We also see a different distribution of citation ideology scores between pages of MPs from the two main UK parties, with Labour MP pages drawing on sources with a slightly higher degree of ideological bias. To further investigate these findings, we contacted experienced editors from the sub-community of Wikipedia curating pages of UK MPs. One possible explanation for this polarisation of sources is that, before election, Labour MPs tend to be less well known than Conservative MPs, and thus only left-wing press tend to cover them when they are nominated. This evidence of polarisation therefore might not necessarily imply political bias, but further research in this direction should  investigate the neutrality of the content coverage in those articles.
    %\item The quality of pages varies from pages which are at a very basic stage of development to manually inspected featured articles. Additionally we see that, on average, more than 50\% of each page covers political and parliamentary career along with almost a quarter covering early life and career. %removing this for now as not super interesting

\textbf{High Source Quality.} In terms of verifiability and information quality, we find that MP articles are generally well sourced, with an average of only 10\% of sentences detected as missing citations. The citation quality is therefore very high overall, similar to Wikipedia medical articles, with sections on early life and career having the highest proportion of statements which lack citations. This suggests that, despite signals of polarisation among contributors, the information in Wikipedia articles is backed by a sufficient amount of sources. Our study finds that the UK Parliament's website is the source of (6\%) of citations on these pages. Official sources like this can be used to improve quality and trustworthiness, although they will not provide effective sources for aspects such as early life and career.



% \textbf{Political implications}
% Through the study we understand the dynamics of engagement and availability of information on MP pages in the UK. We see Wikipedia as an important channel for broadcast political communications with selective enrichment of agreed information content. Our study finds that the UK Parliament's website is the source of (6\%) of citations on these pages. Official sources like this can be used to improve quality and trustworthiness, although they will not provide effective sources for aspects such as early life and career. Conversely, parliament and other platforms can make use of dataset from Wikidata to use crowd-sourced knowledge for their reports. Similar to other online platforms, it is now also important to flag any online hate content on these pages. We will make the results of the survey available to help communities of editors improve the pages.


\textbf{Limitations and Future Work} In this paper, we do not investigate the  dynamics of page evolution over time. We use the final stable page state as of 28th Aug 2019 to compute metrics and features for the content and time patterns. Future work should focus on mining temporal patterns of engagement, including changes resulting from the recent 2019 general election and presence of pages in multiple languages~\cite{hale2014multilinguals,agarwal2020characterising}. %Geo-location is for a subset of edits based on all IP locations we capture from user names. Additional location data is needed to generalise the constituency engagement for each (logged-in) user and if there is a single user with different usernames.
Also, while we trace quality patterns across different topics, we do not look at the value of individual contributions, which could be used to help identify spam and vandalism and thereby measure online hate or disinformation campaigns. %Further, break down of page content into sections is required to quantify readability of sections within pages, thus enabling to further understand and improve content targeting for MP Wikipedia pages. %We will also include in our future work a focus around the 2019 general election and candidates' use of Wikipedia before they become an MP.  

%\textbf{Acknowledgments} We thanks participants of the survey. Additional credits we will add in the camera ready version of this paper.

==> HT Arxiv/sections/dynamics.tex <==

\section{Spatio-temporal patterns of Pages}\label{sec:dynamics}

We begin by investigating when the MPs' Wiki pages are created and edited and
what events or actions have impact on page views. In summary, we find that most MP pages are created soon after they are first elected; edits happen after significant changes such as elections or scandals; and most views happen just before or after important events such as referenda, elections and scandals.





%Table~\ref{table:pagesDate}


% \begin{figure}
% \centering
%   %\includegraphics[width=0.9\columnwidth]{figures/mapEdits.png}
%   \includegraphics[width=0.9\columnwidth]{figures/constiCDFMap.png}
%   \caption{Constituency engagement based on the fraction of edits from each MP's own constituency. Inset: All Edits counts from constituencies of  Greater London area. }~\label{fig:map}
%   \vspace{-0.5cm}
% \end{figure}

% \begin{figure}
% \centering
% %   \includegraphics[width=0.9\columnwidth]{figures/pageCreation.png}
% %   \includegraphics[width=0.9\columnwidth]{figures/positionYear.png}
%   \includegraphics[width=0.8\columnwidth]{figures/postisionAndCreation.png}
%   %\includegraphics[width=0.9\columnwidth]{figures/postisionAndCreationCDF.png}
%   \caption{Counts of page creation (right bar) and first position held (left bar) as an MP.}
%   ~\label{fig:pageYear}
%     \vspace{-0.5cm}
% \end{figure}


% \begin{table}
%     \centering
%     \caption{Percentage of MPs page creation.}
%     {\small 
%         \begin{tabular}{p{2cm}p{2cm}p{2cm}} 
%             \toprule
%             Party	& After wining & Before wining\\
%             \midrule
%             Conservative& 72\%&28\%\\
%             Labour& 73\%&27\%\\
%             SNP& 88\%&12\%\\
%             Others& 42\% &58\%\\
%             \bottomrule
%         \end{tabular}
%     }
%     \label{table:pagesDate}
% \end{table}

% \begin{figure}
% \centering
%   %\includegraphics[width=\columnwidth]{figures/viewsMPActPlay.png}
%   \includegraphics[width=\columnwidth]{figures/viewsMPActPlay.pdf}
%   \caption{Page views of MPs pages. As a baseline we add professional sports people (footballers) and  actors in the UK. The two black vertical lines correspond to 2016 Brexit referendum (left) and 2017 general election (right) results date.}~\label{fig:views}
%     \vspace{-0.5cm}
% \end{figure}


\subsection{Page Views}
Using edit history for each article, we obtain the article creation date (i.e. the day when the first edit was made).  The edit history data covers four UK general elections (2005, 2010, 2015 and 2017). We see from that for the majority of pages, the creation date is close to a general election (60\% of page creation falls within these four years). In addition, 25\% of the articles were created between 2002 and 2004 (both included), coinciding with the birth and subsequent rapid growth of Wikipedia.
We focus on the dynamics of viewing behaviour. MP pages obtain a large number of views, with an average of 247k views per MP during the period we consider. %The per day page view count of any Wikipedia article are available using Wikimedia's public API\footnote{\url{Documentation:  wikitech.wikimedia.org/wiki/Analytics/AQS/Pageviews, Accessed on 28 Aug 2019}}. F
%The earliest date of view count through the API can be 01 July, 2015. The total views in four years duration across all 650 MPs are 160.3 Million. 
We show the average view count of each day (mean) and median in Figure~\ref{fig:views} (Note: Y axis is log scale). The mean views count is high on days of two major events: the \emph{UK EU membership referendum} (also known as the `Brexit' referendum) of 24 June 2016 and the \emph{UK general election} of 09 June 2017. %We find that for total views across MPs the mean is 247k, median is 80k and maximum is 14.5 Million for \emph{Theresa May MP} who was also prime minster of the UK from 2016 to 2019. 


We note from Figure~\ref{fig:views} that near the Brexit referendum there are multiple viewership peaks. This relates to a major reshuffle of government ministers, which took place after Theresa May became the UK's new prime minister. This is similar to the patterns exposed in ~\cite{gobel2018political} for German MPs, where highest views generally follow ministers' resignations and new appointments.
During the \emph{UK general election} we see that the number of views rises from the day of the election announcement~\cite{election2017}. 




Apart from events where a majority of MP pages get attention, there are events which are specific to individual (non-popular) MPs when they are in the limelight. Examples include anticipated and unanticipated events, such as ministers' resignations, speeches, interviews etc.~\cite{agarwal2019tweeting}.
%We find that there is a high correlation (Pearson's correlation coefficient of 74\%, $p<0.001$) between the number of views to MP Wikipedia pages on a given day and the numbers of daily mentions obtained by MPs according to data shared by~\cite{agarwal2019tweeting}. %On Twitter, the average mention count is 70 per MP per day. On Wikipedia we find that on an average MPs get 180 views per day. 
%To correlate the attention on MPs' Wikipedia pages with other social media we use sixty days' dataset of Twitter load from~\cite{agarwal2019tweeting} and correlate views of MPs' Wikipedia pages. %In Figure~\ref{fig:views60} we show mean and median for views on Wikipedia and mentions on Twitter for a period of 60 days across all MPs. 
%On Twitter, the average mention count is 70 per MP per day. On Wikipedia we find that on an average MPs get 180 views per day. %Median views on Wikipedia has high (74\%) \emph{Pearson} correlation with median mentions on Twitter for MPs (p<0.001). %\nishanth{Loads of stats are being computed. But without the "why". You need more of a motivation.}

%only as text
% \begin{figure}
% \centering
%   \includegraphics[width=0.9\columnwidth]{figures/mentionsViews60.png}
%   \caption{We show here mean and medians of views on Wikipedia and mentions on Twitters across all MPs.\pushkal{Optional.} }~\label{fig:views60}
% \end{figure}

\subsection{Page Edits and their Spatial Distribution}
Another core dimension of engagement with Wikipedia is the editing process carried out by largely anonymous volunteers. %We analyze here the edit history for the 650 MP pages. 
Among all edits, 36\% happen during the last three election years captured in the dataset (2010, 2015 and 2017). These patterns are similar to the views pattern in Figure~\ref{fig:views} (Pearson's correlation: 62\%, $p<0.001$), and we omit the figure with daily edit counts due to limited space. 
%In total, there are 231k edits since 24 June 2002 (creation of the first Wikipedia page for Boris Johnson) until 28 Aug 2019. %We also see that majority times 155k (67\%) there are new additions by editors. 
%\nishanth{As mentioned, we really need a good reason why we stop before the 2019 elections.. Perhaps it is too fresh and the numbers of views etc may not be fully captured in the few months since the election?? And we should not be saying last three elections (that is factually incorrect), but rather "the three elections captured in the dataset"}\pushkal{updated text for three election years. For dataset, yes 2019 is quite new}
%The mean number of edits per MP article is 356, median is 222 and maximum is 8.5k for current prime minister \emph{Boris Johnson MP}. %He is also the one who got first page edit across all MPs in our study (June-2002).
%In total there are 43k unique editors who have edited UK MPs article on average 5 times (median is 1). Taking the unique editors count for each MP page we find that the median number of editors for each page is 117 and the maximum is 3k, again for \emph{Boris Johnson}.  %The top (6141) contributions to these pages are by a user \emph{Philip Cross} \footnote{\url{www.bbc.co.uk/news/blogs-trending-44495696}} and second highest edits by \emph{BrownHairedGirl}\footnote{\url{User accessed as on 16 Feb 2020: en.wikipedia.org/wiki/Template:Adminstats/BrownHairedGirl}} whose edits so far on Wikipedia are 1.6 Million. 

%\subsection{Spatial Distribution of Edits}
Out of all the edits, around 55k (22\%) edits are by public IPs which are recorded in the page revision history for not logged-in (anonymous) users. %These IP addresses are stored publicly after notifying the editor can be seen directly in the page revision history. 
To understand the spatial distribution of editors, we map each public IP to a possible physical location (postcode), %For public IP edits we locate the editor 
using the service provided by \emph{db-ip.com}, a geo-location database.
%\footnote{IP geo-location and database by db-ip.com, Accessed on 18 March 2020}
We observe that 84\% of public IP edits are from the UK. The remainder are from countries such as the United States--1768 edits, Ireland--442 edits, Australia--364 edits, Canada--297 edits, etc.% and so forth.

We then map each postcode to a local constituency using the list provided in~\cite{agarwal2019tweeting}.  We plot edit location at constituency level in Figure~\ref{fig:map} (inset), and observe that most public IP edits come from the area of Greater London, and more specifically from the Westminister borough (318 edits) where the Parliament sits. This is indicative of MPs' staff managing edits, similar to the findings of previous studies, which could provide a source of bias in the articles~\cite{gobel2018political}. % After labeling local constituency for the editors, 
The highest number of public IP edits coming from an MP's local constituency is for MP \emph{Amber Rudd MP}, former home secretary, who has 47 out of 232 edits from her own constituency (Hastings and Rye). %Other top MPs are \emph{Rachael Maskell} (21/28), MP \emph{Royston Smith} (19/25) and so forth. 
%Looking per constituency edits we find that the highest edit (318) are from \emph{Cities of London and Westminster} constituency. This is an indicative of MPs staff managing edits similar to study in~\cite{gobel2018political}. In general there are more edits from Greater London area which we show Figure~\ref{fig:map} (left).

To further quantify the extent to which edits come from an MP's constituency, we calculate the \textit{Constituency Engagement Factor (CE)} of each MP $m$ as the proportion of the edits to their articles which are localised to their constituency. If $m$ has $N_{m}$ edits of their page and $N_{m,c}$ edits from their constituency, we write: 
\begin{equation}\label{eq:localengagement}
    CE_{m,c} = \frac{N_{m,c}}{N_m}
\end{equation}
We plot the distribution of the metric in Equation~\ref{eq:localengagement} in Figure~\ref{fig:map}. We see that for 31\% of MPs there is at least one edit from their own constituency, but $CE$ is in general low, and only 6 MPs have more than half of their edits from their own constituency. 


%\pushkal{Add text for the chart.}
%\pushkal{ We are not covering in this deletions, edit wars, bot edits etc.. It is reported by past studies that these are not significant in MPs pages. ~\cite{graham2015digital} to
%add factors such as internet availability, population etc. LATER}

%We next section we discuss the interest of editors while editing MPs pages.


==> HT Arxiv/sections/introduction.tex <==
\section{Introduction}

% Commands:
% \pushkal{Pushkal}
% \nishanth{Nishanth}
% \miriam{Miriam}
%\pushkal{Notes: Use date format as 23 Feb 2020, we use Wikipedia article or Wikipedia pages as interchangeably, ... }

%\pushkal{Removing: Reading score and  Ores article quality sub-section.-- Moving citation quality to polarisation.--Shortening survey.--Moving text to appendix.-- Use ``'Polarisation'' wherever applicable.}

Political communication is defined by Brian McNair as ``purposeful communication about politics''~\cite{mcnair2017introduction}. It includes (inter alia) communication about politicians and other political actors, and their activities, as contained in news reports, editorials, and other forms of media discussion of politics such as large-scale online encyclopedias like Wikipedia.  %The mass media includes print, broadcasting and the internet. 
%In a liberal democracy, knowledge and information must be freely available to all as the basis on which citizens make informed decisions.
Information about politics on Wikipedia would appear to fulfil at least three of the functions of the communication media in `ideal-type' democratic societies as described by McNair: informing citizens of what is happening around them; educating as to the meaning and significance of the `facts'; and publicising the activities of governmental and political institutions~\cite{mcnair2017introduction}. 
%\pushkal{Edward delete: As early as the 1960s, commentators became interested in the idea that networked communicators could facilitate greater direct participation in political processes by members of the public. Some have been enthusiastic about this prospect, regarding it as democratically beneficial~\cite{blick2020electrified}. Others have held can bring with it problems, for instance by promoting `populism', however defined. The rise of the Internet as a mass-use phenomenon from the 1990s has not led, in the UK or elsewhere, to continuous electronic referendums. However, it has changed the way in which politicians within the representative system and members of the public interact, for instance via social media and online petitions and consultations. It has also raised various difficult questions regarding how these digital technologies should be regulated, to ensure that they do not contaminate or destabilise political processes.\pushkal{Edward: The introduction is too much about direct citizen participation in politics.  This may apply to Wikipedia MP articles to some extent but there are other ways to explain the phenomenon, eg.
%1) classic political communications (broadcast) using a new medium which makes it much easier to put information into the public domain and reach potentially millions of people
%2) citizen participation in civil society through editing Wikipedia pages -- how different are editors of MP pages different from Wikipedia editors generally?
%Wikipedia is one such major source of information that provide large variety of content online.
%}
%}

Wikipedia's political content is pretty extensive. For example, all 650 elected  Members of the Parliament (MPs) in the United Kingdom (UK) %from House of Commons 
have a Wikipedia page or article\footnote{We use the terms `page' and `article' interchangeably. The dataset we collected from these articles is available for the research community here: ~\url{tiny.cc/wikipedia-mps}}. Such content is also widely reused by the broader web: due to the popularity of Wikipedia as a platform, the top results returned by search engines queried for MPs show links to their Wikipedia pages. %Political actors may therefore regard Wikipedia as an attractive platform for advertising elected representatives and candidates by controlling the information flow or enhancing their image~\cite{gobel2018political}.  %Often, there is also an information panel (mostly on the right side) that curate information from the Wikipedia.  
%Wikipedia pages of high profile people such as politicians are widely viewed. 

Given the visibility of Wikipedia, and the importance of the online encyclopedia in forming public opinion, the integrity and completeness of its content is crucial, especially % edits which are made 
during ``times of shock''such as elections or referenda ~\cite{zhang2019participation,10.1145/1240624.1240698}. To ensure information quality, Wikipedia editors operate in compliance with the core content policies of Neutrality and Verifiability\footnote{\url{https://en.wikipedia.org/wiki/Wikipedia:Core_content_policies}}. However, the scale of information and the free-to-edit Wikipedia policy sometimes limit the capability of communities to maintain the quality and neutrality of Wikipedia pages, and little is known about the life-cycle and quality of Wikipedia articles in the context of politics.



In this paper, we contribute to political communication studies by investigating, for the first time, citizens' engagement with politicians through the lens of the largest online encyclopedia. %More specifically, we are interested in 
%It is important for such pages to have an unbiased content.  Another important concern is to understand what people are actually looking for in Wikipedia articles (we interchangeably use the terms `articles' and `pages') and if the corresponding content is available.
We perform a large-scale quantitative analysis of collective attention, quality, and polarization on Wikipedia pages of Members of Parliament in the UK. To this end, we collect a huge dataset of all edits (231k) and views (160M, since 2015) to UK MPs' Wikipedia articles.
We first investigate the spatio-temporal patterns of readers' and editors' engagement using the 650 UK MPs' Wikipedia articles. To understand the value of the political information viewed by millions of readers every month, and identify potential biases in political content in Wikipedia, we next focus on the \textit{polarisation} of MP pages' editors and citations% typically MP staff, party volunteers and regular Wikipedia editors ~\cite{gobel2018political}
. To do so, we look at editors' preferences in terms of the political party of the subjects they edit, as well as the overall polarisation of the sources across MP Wikipedia articles, and %, these edits can be from M. Hence, to understand editors preference we characterise \emph{polarisation} as the extend of attachment to a party. 
%This work builds upon the dynamics patterns study by~\cite{gobel2018political}. W We see that MPs pages receive views and edits largely during elections times. It becomes crucial to understand then how large is the \emph{attention load} on Wikipedia during these time, and the organised efforts of page creation and edits. As per~\cite{gobel2018political}, these edits can be from MPs staff, party volunteers and regular Wikipedia editors. Hence, to understand editors preference we characterise \emph{polarisation} as the extend of attachment to a party. 
finally compute at the quality and completeness of the citations in MP Wikipedia articles. %, to which are exposed millions of readers every month. % inWikipedia pages are viewed by Millions of user it is extremely necessary that the information supplied is correct and useful
%Another important concern is to understand is the \emph{quality} of MPs Wikipedia pages. As these pages . We check this using the page content (683k words) and other metadata from Wikidata.org, a free Wikimedia foundation knowledge base.
%To this end, we first perform a quantitative analysis of articles'  reference correctness. %We then run a survey to collect impressions from Wikipedia readers about articles' completeness.
% goodness of a \emph{stable} article if it is well cited, easy to read for a wider audience and covers aspects that user think are important. 
We list these focus areas in the following research questions:

\noindent\textit{\textbf{RQ-1} What are the spatio-temporal patterns on MPs Wikipedia pages?}  Are there times of heavy edit and pageview loads?
(\S\ref{sec:dynamics})

\noindent\textit{\textbf{RQ-2} What is the quality of edits and citations on these pages? }
Is there polarisation of edits and citations along party lines? What is the citation quality?
(\S\ref{sec:polarization})

% \noindent\textit{\textbf{RQ-3} What is the quality of these pages and their sections? Are some pages more readable than others?} (\S~\ref{sec:quality})

%\noindent\textit{\textbf{RQ-3} Are these articles complete and useful for citizens? What do people think based on a survey?}
%(\S~\ref{sec:usability})

We find that engagement with MP Wikipedia articles is synchronized with election periods, and that  a mild form of polarisation exists in editors' preferences and article references. Furthermore, we verify that citation quality is generally high.
%, while articles' complexity makes them accessible (readable) only to college graduates. Despite observing that  overall article quality is below average, 
%Our survey finds a general alignment between readers' information needs and MP article content, showing that editing dynamics are successful in creating an effective corpus of content.

Collectively, these findings contribute to an in-depth understanding of political communication via Wikipedia. We discuss potential implications for information quality monitoring and disinformation studies in \S\ref{sec:discussion}.
 
% With these set of questions we shed light on online engagement and quality of politicians' pages. We make the following contributions: 
% \begin{itemize}[leftmargin=*]\itemsep0em
%     \item We explore spatio-temporal patterns including geo-located constituency edits.
%     \item We further quantify the gaps and bias in the articles. We do this by checking partisanship of news and communities of editors. 
%     \item We devise and compute quality metrics across party and gender lines, and further correlate characteristics of good articles.
%     \item Finally, from the responses of around 60 participants we identify users' needs and make recommendations for the content of MPs' Wikipedia pages. 
% \end{itemize}

%In the rest of the paper, we first provide background and describe related work from this area of study. Then we list details of our carefully collected and processed data. Then there are sections based on research questions we list above. Finally, we conclude with a discussion which also covers our future work and limitations.

==> HT Arxiv/sections/polarization.tex <==
\section{Polarisation and Quality}\label{sec:polarization}


%In this section we investigate how editors prefer certain pages over the others. We also present for MPs pages the association with different categories and gaps.
We continue our study by looking at information quality through the lenses of potential ideological and societal biases in Wikipedia articles about UK MPs. We ask and answer two questions: \textit{(i)} Do editors have an ideological bias, e.g., focusing on editing pages of MPs from a specific party? \textit{(ii)} What is the quality of citations used for MP pages? Do they have an ideological slant, and is their coverage sufficient? We find that there is a specialisation of editors, with some focusing mainly on Conservative party MPs, others on Labour MPs, and so on. %Similarly, we find that there is a small but significant ideological leaning among citations -- Labour MP pages contain citations from left-leaning news papers whereas the Conservative MP pages are supported by citations from right-leaning news papers. %First, we quantify the amount of ideological polarization across 
%\pushkal{We present quality of citations of these pages and find that topic like early life and career are hard to cite and hence miss citations.}


\subsection{Editors' Ideological Preference}
%Given that the total count of edits history on MPs pages is now in six digits, it is interesting to see what preferential attachment exists. 
To understand the extent to which editors tend to polarize around a specific ideology, we start by tracing, for each of the 42k editors, the party of pages which they mostly edit.
To this aim, we compute the number of edits to MPs from a given party, similar to~\cite{barbera2015birds,agarwal2019tweeting}, and associate each editor to the party to which they contribute the maximum edits. %For example, if an editor edits more than half of the times unique MPs from Conservative (Labour) party, then we label an editor as Conservative (Labour) editor.
We do this for editors editing at least three different MPs, in order to exclude cases in which an editor is %. We do this to remove cases where an editor is 
only interested in one MP or two MPs from different parties. This filtering step leaves us with 4.2k (7\%) of editors who are collectively responsible for 67\% of edits. % or there is a conflict between two MPs each of which is from a different party.
%From 4.2k  \pushkal{check} editors which are left after filtering, with this model 
%After assigning party preferences to editors we see that 62\% of editors favour Conservative MP edits with 31\% favouring Labour, 2\% SNP and 5\% other parties. When we normalise this with total MPs per party we see that the Conservative party has 8 editors per MP against Labour which has 5. The count for the SNP is low with 2 editors per MP. 

% \begin{figure}
% \centering
%   \includegraphics[width=0.54\columnwidth]{figures/crossPartyNoOne.PNG}  
%   \includegraphics[width=0.45\columnwidth]{figures/editsJacc5.png}
%   \caption{Left: Cross-party edits. Right: Network graph based on co-occurrence of MPs for each editor. }~\label{fig:crossParty}
% \vspace{-0.5cm}
% \end{figure}
% \begin{figure}
% \centering
%   \includegraphics[width=0.8\columnwidth]{figures/ideology.pdf}
%   \caption{Ideology scores and density.}~\label{fig:ideology}
% \vspace{-0.5cm}
% \end{figure}

\begin{figure}[thb]
    \centering
    % \subfloat[Cross-party] {
    %     \includegraphics[width=0.30\textwidth]{figures/crossPartyNoOne.PNG}
    %     \label{fig:crossPartyHeat}
    % }
    \subfloat[Editors Network] {
     \includegraphics[width=0.4\columnwidth]{figures/editsJacc5.png}
    \label{fig:crossPartyNet}
    }
    \subfloat[Ideology scores] {
    \includegraphics[width=0.57\columnwidth]{figures/ideology.pdf}
    \label{fig:ideology}
    }
    \caption{Measure of Polarisation (Red: Labour, Blue: Conservative, Black: Others). %(a) Edits from each Party editors (rows) to UK MPs pages (columns).
    (a) Network graph based on editors as nodes, with edges connecting editors who have edited the same MPs' pages. (b) Ideology scores and density based on citations domains.}
   % \vspace{-0.5cm}
\end{figure}


To understand communities forming this polarisation we perform network analysis -- %We compute network-based metrics to check similarity in edits and communities of editors. %In other words, to what extent are there communities of editors editing the same MPs' pages. 
 we define editors  as nodes and induce weighted edges between each pair of editors by computing the \emph{Jaccard Coefficient} or similarity of the sets of pages edited by them. Thus, if two editors
%\footnote{\url{www.statisticshowto.datasciencecentral.com/jaccard-index/}}
edit exactly the same set of MP pages, the weight will have its highest value of 1, and if there is no overlap, the value will be 0 (considered as no edge). We then use the Louvain method to identify communities of editors who have more connections within each community, but not many connections across communities. We find that this graph cleaves into 8 tightly knit communities, with a high modularity score of 0.229, indicative of polarisation or specialisation by party among editors. 

To visualise this better, we focus on the most active editors, and remove nodes with a degree of less than 5. To remove clutter, we do not show edges with weights less than 0.5.  Figure~\ref{fig:crossPartyNet} depicts this graph  by colouring the nodes (editors) based on their party (Blue for Conservative editors, red for Labour and black for others), and visually confirms the polarisation detected above by showing how the graph of editors divides along party lines,.  
%We compute the Jaccard coefficient pairs for each in 4.2k users using parallel foreach loop in R on a high performance server. This gives around 9 Million un-directed edges ((4.2k X 4.2k)/2). 
 %We find that the \emph{Number of Communities} formed is 8 with a \emph{Modularity} score of 0.229. This indicates formation of editors communities having more connections within modules but loose connections across nodes of different modules. %\emph{Average Clustering Coefficient} is 0.7 and . 
%We show a small sample of this network in Figure~\ref{fig:crossPartyNet}. For simplicity, the visualisation has edges with Jaccard coefficient of more than 0.5. We also remove isolated nodes and nodes with degree of less than 5. We can clearly see the formation of communities. We run \emph{ForceAtlas 2} model which is well known for visualising communities and induce attraction force on nodes if they have common edges.  The size of nodes is proportional to their degree and edge color is based on the source node.

% \begin{figure}
% \centering

%\includegraphics[width=0.9\columnwidth]{figures/mps100Edits.png}
%  \caption{Network graph based on co-occurrence of MPs for each editor.}~\label{fig:crossPartyNetwotk}
%   \vspace{-0.5cm}

% \end{figure}




\subsection{Citations Preference}
We next focus on the \emph{content} rather than the authors. We may expect that if authors exhibit polarisation, the sources they draw from to write the content, i.e., the MP pages, may also be polarised. To quantify this, we use URLs which are embedded in the \emph{References} section as citations. We find that there are 19k citations on MP pages. The average citation count is 29 per page and the median is 19. By checking the top citation URLs, we see that majority of them are news domains. This is consistent with the English Wikipedia articles study by~\cite{piccardi2020quantifying} which shows that top domains cited are 
Google.com, DOI.org, Nytimes.com. NIH.gov, BBC.co.uk, TheGuardian.com and so forth. Similar to~\cite{piccardi2020quantifying} we also extract the base domain from each citation URL and obtain 2212 unique domains. Additionally we find long URLs for 1.4k web archive \emph{(web.archive.org and archive.is)} short URLs. The top 5 domains which we get are BBC (15\%), theguardian (11\%), telegraph (6\%), parliament.uk (6\%), independent (5\%). The top 10 domains cover 52\% of the citations list. %All of these top sources are either news domains or official publishers such as the UK Parliament.

To check the use and representation of news domain sources on MP pages we compute an ideology score for each MP page. To do this we first check and label all possible news domains with their political leaning. We use scores from \emph{Mediabiasfactcheck}~\cite{mediaBias} and label the top 50 news domains with their political leaning (left, center or right). We also add ideology scores for news domains using sub-strings such as conservative (right-leaning) or labour (left-leaning) in the domain name. With this approach we find and label 67\% (13k) of the domains. %Table~\ref{table:domains} shows some examples of the top domains we label with the total citations count. 
Some examples of top domains by citations count are Left--Theguardian (2069), Independent (969), Newstatesman (262); Center--BBC (2766), Parliament.uk (1151), UKwhoswho (233); and Right--Telegraph (1207), thegazette (302), thetimes (251). 
%The most cited page is from a Spectator article on which Conservative MPs support Brexit (bit.ly/2JtcvkW).


% \begin{table}
%     \centering
%     \caption{Examples of domains from each category.}
%     {\small 
%         \begin{tabular}{p{1cm}p{6.5cm}} 
%             \toprule
%             Type	&	Top domains (Citations count)	\\
%             \midrule
%             Left		&
%             Theguardian (2069), Independent (969), Newstatesman (262) \\
%             \midrule
%             Center	&
%             BBC (2766),
%           Parliament.uk (1151),
%             UKwhoswho (233)
%             \\           \midrule
%              Right	&
%             Telegraph (1207),
%             thegazette (302),
%             thetimes (251)
%             \\
%             \bottomrule
%         \end{tabular}
%     }
%     \label{table:domains}
%     \vspace{-0.5cm}

% \end{table}


After labeling, we compute an ideology score for each page, as the fraction of identified and \textit{Mediabiasfactcheck}-labelled news domains on that page that are left-leaning (i.e., ideology score = (number of left leaning news domains in citations)/(number of left+right leaning citations)). Note that a score of 0 indicates usage of only right-leaning sources and a score of 1 indicates only left-leaning sources; a score of 0.5 indicates a perfect balance.  Figure~\ref{fig:ideology} shows the ideology scores of Conservative and Labour pages as scatter and density plots. We see two peaks (median Labour: 0.7 and median Conservative: 0.4) which indicate a slight polarisation, with a slightly more polarised (i.e., farther away from 0.5) score for Labour MP pages. Also, 53 (17\%) Conservative and 57 (22\%) Labour pages have extreme polarised scores of 0 and 1 respectively. The KS statistics test (two sample) also confirms that there is a significant difference ($p<0.001$) with a distance value $D=0.54$ in the two parties' ideology scores. 
%\pushkal{Edward: on the x axis, is 0.0 zero bias and 1.00 total bias?
%In the text, I think you should describe clearly the finding that Labour MP articles are more biased than Conservative ones.}
%\pushkal{Added now.}
% \subsection{Back-links clusters}
% UK Labour MPs page have link to labour MPs, etc.

\subsection{Citation Quality}
%On Wikipedia, the first (or main) section on each page is a summary section, which is mostly followed by a table of contents, then there are sections and at the end citations.
To further understand the quality of Wikipedia articles, we perform an additional experiment on citations,  a key element for monitoring information quality in Wikipedia. % The Wikipedia core content policy of Verifiability requires that most material is backed by a reliable source supporting the information.
Are MP articles well sourced? To answer this question, we compute a citation quality score for each page. %We use page content to compute the citation score of pages. For this w
To this end, we employ the ``Citation Need'' model defined in ~\cite{Redi:2019:CNT:3308558.3313618}. The model takes as input a sentence in a Wikipedia article and assigns a Citation Need score $s_{cn}$ in the range $[0,1]$. The higher the Citation Need score, the more likely it is that the sentence needs a citation.

\begin{figure}[th]
    \centering
     \includegraphics[width=0.9\columnwidth]{figures/missingCitationBar.png}
 \caption{
Percentage of sentences which miss citation.}
\label{fig:citation}
%\vspace{-1cm}
\end{figure}


For each article we first parse all sentences and score them with the Citation Need model, after  filtering out statements in the  main section, which are less likely to need a citation%'s statement which are most cited somewhere else in the paper according to author's writing style
~\cite{Redi:2019:CNT:3308558.3313618}. % We obtain 8.8k statements from this filtering and check fraction of citation presence as follows,
Next, we aggregate the sentence-level scores and compute a Citation Quality $CQ$ as the proportion of sentences needing citations that already have a citation. To do so, we first identify the set ${C}$ of sentences needing citations in an article ($N$), namely those sentences whose $s_{cn}$ is greater than 0.5. Next, we count how many sentences in the set ${C}$ already have a citation in the original article text ($N_c$). Finally, we compute citation quality as the ratio between these two quantities:
\begin{equation}
CQ=\frac {N_c}{N},
\end{equation}

%compute the percentage of sentences classified as needing citations 
%In total we have 11.5k paragraph statements. %The mean (and median) of statements per MP is 18 (and 14). Out of these, 1.6k (7\%) do not have any citation. 
%We show citation scores for both statements type, which have citation and those which do not have citation in Figure~\ref{fig:citationCDF}
%To compute the quality of page citation we check for statements which needs citation has (or has not) a citation. 
%To do this we take statements with citation needed score greater than $0.5$ (86\%). Additionally we 
%%
%$$
%citationQuality = \frac{|statementsCited \cap statementsNeedCitation|}{ |statementsNeedCitation|}
%$$
We check the distribution of citation quality values for each party. %(\pushkal{Note: We omit the CDF plot due to lack of space and non-significant differences})
We see with the KS statistics test that for all party pairs there is no significant difference. However, we see that some pages for all parties have values of less than 0.5. We manually check these pages (50) and find that they are mostly in the Stub, Start and C (has significant problems) quality categories.
%\pushkal{Miriam will check and add more stats from MPs pages who have less citation score.}

We see that the average citation quality for MP articles is pretty high: about 83\% of sentences needing citations actually have one. This is higher than the average citation quality in English Wikipedia, and comparable to articles about Medicine and Biology, which historically are constantly monitored for information quality \footnote{\url{meta.wikimedia.org/wiki/Research:Mapping_Citation_Quality}}.
We see that citation quality is uniform across MPs from different parties.
%For highest, we see MP Rehman Chishti page statements need citation. This is significant for him possibly because his awards given subsection statements lack in citations. From the section view of missing citation, MAIN SECTION contributes to 26\%,  Parliamentary career to 20\%, Political career 13\% and so forth in decreasing proportion.
Among the articles with high citation quality score we find many with low quality Wikipedia article scores: for example, Scottish MPs David Linden and Martin Docherty, despite having just a few lines in their article (quality ``Start''), have a $CQ$ equal to 1 because of the richness of their citations. Conversely, we find that most articles with low citation quality are also low quality articles, with a few exceptions including the article about MP Robin Walker.
%For the subset of statements which have  citations we see that \url{bbc.co.uk} (11.4\%)and \url{theguardian.com} (8\%)  are top domains which are used for citations which we see in previous section as well. 

We report the percentage of statements where citation is missing in given sections in Figure~\ref{fig:citation}. For instance we see that sentences from \emph{Early Life and Career} miss citations the most often (18\%). It is likely that this section can be hard to find citations for as there may be fewer references in the digital media. We see that Expenses, Political Views, Controversies and Honours are the best cited sections with only 5\%--7\% of statements missing citations.


==> HT Arxiv/sections/quality.tex <==
% \section{Quality of Wikipedia}\label{sec:quality}
% %Taking the word count for each MP page we find that the mean is 1051, median is 736 and highest is 13k for MP and former Labour party leader \emph{Jeremy Corbyn}, showing that MP pages vary significantly in length.\pushkal{This section can be written as a fusion of dynamics and polarisation that relates to good quality pages. For example high viewed pages are good? Polarised groups edit better? etc.} 
% We now move to analyze the quality of MPs' Wikipedia pages. We start by analyzing the quality of content which editors add. We operationalize the notion of quality through existing measures of article quality, citation quality and text readability% to develop an overall measure of quality
% . First, we make use of the ORES Wikimedia API~\cite{ores} to obtain, for each article, a quality score, similar to~\cite{Redi:2019:CNT:3308558.3313618}. For citation quality, we check if a statement needs a citation and if it has a citation or not using the test developed by~\cite{Redi:2019:CNT:3308558.3313618}. Finally, we compute articles' readability using Flesch-Kincaid~\cite{si2001statistical} and other readability scores.
% We provide a detailed explanation of the models used and the quality analysis result in the following subsections.


% %Using a single figure star for all 3 quality plots
% \begin{figure*}[thb]
%     \centering
%     \subfloat[Citation Quality] {
%         \includegraphics[width=0.33\textwidth]{figures/missingCitationBar.png}
%         %\label{fig:citation}
%     }
%     \subfloat[Readability] {
%         \includegraphics[width=0.33\textwidth]{figures/readingPartyMain.png}
%         \label{fig:reading}
%     }
%     \subfloat[Article Quality] {
%         \includegraphics[width=0.33\textwidth]{figures/qualityPrediction.png}
%         \label{fig:quality}
%     }
%     \caption{Dimension of pages quality. (a) Percentage of sentences which miss citation. (b) Reading Grade (RG) of main and page content per party. (c) Prediction of quality category. Darker the shade better is the page quality.}
%     \vspace{-0.5cm}
% \end{figure*}
    
    
% \subsection{Categories and Section}
% %The most frequently seen section headings are in Figure~\ref{fig:sectionTop}. 
% There are in total 11.5k sections on the 650 MP pages, with an average of 4 sections per MP articles (up to 14 for more popular MPs). %We find a total of 392 unique section titles and on average (as well as median) there are 4 sections which can be up to 14 for more popular MPs. 
% To assist our analysis of article quality, we manually group the 392 unique section titles into 12 labels% in two iterations
% , avoiding overlaps in the content covered by different labels as far as possible. The label with the highest percentage of words in relation to overall article length is \emph{Political and Parliamentary career} (56\%) which includes section headings such as Parliamentary career, Member of Parliament, House of Commons etc. Next we have \emph{Early life and career} (18\%) which includes section headings such as History, Education, Background, Early Career, etc. Other major labels are Main section (10\%), Personal life (6\%), Political views (5\%) and the rest cover the remaining 5\%. 

% To explore potential content biases, we breakdown section statistics party. %To understand whether at section level, take MPs' party and gender and ask if contributions to sections vary in size across these two categories.
% We compute the number of words for each section label, and aggregate over all articles of MPs of specific party (for example, we take the average number of words in Main Section of Conservatives and compare with the Main section of labour MPs, etc). %\pushkal{Paragraph updated. Need to add text based on Edward's comment here. EW: paragraph updated, let me know if i've got it right!}.
% To check significant differences in word count we perform the ANOVA test
% %\footnote{\url{www.sthda.com/english/wiki/one-way-anova-test-in-r}}
% on the resulting label distributions. %ased on average number of words for each category for each label type (for example, taking the average number of words in Main Section of Con:female, Lab:Female MPs, etc). 
% We get significant differences across categories for each of the three main labels -- Political and Parliamentary career ($p<0.001$), Early Life and Career ($p<0.05$) and Main Section ($p<0.001$). The distribution between political career and early life is different for each of the three main parties. In particular Conservative MPs' pages have slightly more about political career and less about early life as compared to Labour MPs. 
% %For Conservative, female MPs' pages have more about political career and less about early life than male MPs, whereas for Labour MPs, the distribution is similar for both male and female MPs. %For Labour, female MPs have more about political career, but less about early life than male MPs.
% %\pushkal{Removing plot of categories and section stacked bar. This is covered in text.}

% % We see from Figure~\ref{fig:partyGenderReference} that for SNP MPs, the main section comprises a larger fraction of the page. This is indicative of the rest of the page containing less detailed information in other categories such as political views and (in the case of female SNP MPs) political career. %We next see female MPs from SNP and others have less proportion of Political and Parliamentary career. A possible reason could be that female MPs are represented more in the Parliament in recent year elections than previously and hence have less records\footnote{\url{en.wikipedia.org/wiki/Women_in_the_House_of_Commons_of_the_United_Kingdom}, Accessed on 16 March 2020}. \pushkal{We need to add more details from new figure now.} 

% % \begin{figure}
% % \centering
% % %\includegraphics[width=\columnwidth]{figures/sectionPartyWordsBar.png}
% % \includegraphics[width=\columnwidth]{figures/sectionPartyWordsBar12Cat.png}
% % \caption{Stacked Bar plot of words count in section for each party and gender pair.
% % }~\label{fig:partyGenderReference}
% % \vspace{-0.5cm}

% % \end{figure}



% \subsection{Readability}
% %One way of specialisation can be a writing style. 
% The next dimension of quality we analyze is readability of articles. We compute this as reading grade of the article's body, and its main section.
% %As expected, we find that the main section  is easier to read than the article's body. We find that median Flesh \miriam{How does this compare to the rest of the Wikipedia?}
% We use a method similar to ~\cite{brezar2019readability} to compute Reading Grade ($RG$) which is the near equivalent of reading age. This involves computing the average of 
% Flesch--Kincaid ($FK$),  Simple Measure of Gobbledygook ($SMOG$) and Gunning Frequency of Gobbledygook ($FOG$) scores.~\cite{si2001statistical,benoit2018quanteda} We compute these after removing links, punctuation (except `.' and `,') and references to citations using R package~\cite{benoit2018quanteda}. We formally define Reading Grade ($RG$) as follows:

% \begin{equation}
%  RG=\frac{FK+SMOG+FOG}{3}
% \end{equation}
% %\ns{is this your definition? If so, why is taking a mean of the three scores useful? And are they all on the same scale from 0-100? If not you cannot just merge them in a linear fashion. }\pushkal{We use this formula from~\cite{brezar2019readability} as stated above.}
% We plot $RG$ of main section and page content of each MP page in Figure~\ref{fig:reading}. We see that main sections (median $RG=15.55$) are easier to read than page content ($RG=18.15$). In~\cite{brezar2019readability}, the authors report that the average $RG$ of the twenty-five most-viewed Wikipedia pages on diseases is 12.73 (sd: 0.32). This shows that over the years disease pages become easy to read with high and significant correlation between $FK$, $SMOG$ and $FOG$. They categorise $RG$ scores as under 12--fairly difficult (High school), 12 to 14--difficult (College level) and above 14--very difficult (College graduate level). We check percentage of main section and page content of MP articles based on this categorisation. We find that the main section of 9\% of pages are fairly difficult, 21\% are difficult and 70\% are very difficult. For overall page content 0.6\% of pages are fairly difficult, 1\% are difficult and the rest 98\% are very difficult. %\pushkal{Are we interested in knowing what are these difficult sections of the page content? EW: It would be more interesting to know why the pages are so difficult, but that will have to wait for another paper!}

% We also break down the $RG$ score by party, and find that Labour and SNP pages are easier to read than Conservative (KS-stats: (Con, Lab) D=0.16 and p<0.001, (Con, SNP) D=0.34, p<0.001). We show per party distribution in Figure~\ref{fig:reading}.%\pushkal{These numbers are distance in the distribution and if that if significant or not.}


% \subsection{Article Quality}
% The ORES~\cite{ores} API computes the probability of an article belonging to a given quality category  based on page length, infobox, number of images, sections etc. Given an article, ORES returns 6 probability scores, one for each quality level (\textit{Start, Stub, C-level (C), B-level (B), Good Article (GA), Featured Article (FA)})\footnote{More info- \url{en.wikipedia.org/wiki/Wikipedia:Content_assessment\#Grades}}.

% In Figure~\ref{fig:quality} we show the average quality score for each quality category, broken down by MPs' parties. %(known as \emph{articlequality}) which we use from Wikimedia API  which is a \emph{drafttopic} classifier~\cite{  asthana2018few,Redi:2019:CNT:3308558.3313618}. Similar to~\cite{halfaker2017interpolating, Redi:2019:CNT:3308558.3313618} we use ORES's \emph{articlequality} model which predict level of quality of an article
% %In Figure~\ref{fig:quality} we shows the predicted category based on eight quality categories provided by ORES. 
% Darker shades correspond to better page quality labels.
% We observe two major trends. First, despite the high overall citation quality, the quality of articles is largely poor: the majority of the articles for all parties are marked as ``C-level'', namely articles which are substantial but are  ``still missing important content or may still have significant problems which require substantial cleanup''.
% Second, we observe that articles on Conservative MPs tend to be of overall higher quality. To test if this is statistically significant %Additionally 
% we perform the ANOVA test, by converting quality category labels to numerical values such that 0 is Stub and 5 is Feature Article.  We find that there is a significant difference ($p<0.001$) in the ratings of articles across parties.

    
% % \begin{figure}
% % \centering
% % \includegraphics[width=0.8\columnwidth]{figures/qualityPrediction.png}
% %   \caption{Prediction of quality category of page. Darker the shade better is the page quality. }~\label{fig:quality}
% %   \vspace{-0.5cm}
% % \end{figure}
% % \begin{figure}
% % \centering
% %   \includegraphics[width=0.9\columnwidth]{figures/missingCitationBar.png}
% %   \caption{Percentage of sentences which miss citation according to citation needed scores.}~\label{fig:citation}
% %   \vspace{-0.5cm}
% % \end{figure}
% % \begin{figure}
% % \centering
% % %  \includegraphics[width=0.9\columnwidth]{figures/readingScore.png}
% %   \includegraphics[width=0.9\columnwidth]{figures/readingPartyMain.png}
% %  % \includegraphics[width=0.9\columnwidth]{figures/readingPartyMainFS.png}
% %   \caption{Reading Grade (RG) of main and page content per party. }~\label{fig:reading}
% %   \vspace{-0.5cm}
% % \end{figure}





% % UK population as per
% % \url{https://www.ons.gov.uk/peoplepopulationandcommunity/populationandmigration/populationestimates/articles/overviewoftheukpopulation/february2016} in 2014 Population aged
% % 0 to 15 (18.8\%), Population aged
% % 16 to 64 (63.5\%), Population aged 65
% % and over (17.7\%).

% % % https://www.syssec.ruhr-uni-bochum.de/media/emma/veroeffentlichungen/2019/09/05/uninformed-consent\_Yl7FPEh.pdf
% % % Emergent thematic coding

% % % Two of the authors independently devised a set of codes for each
% % % question and coded the responses. The results were discussed and
% % % yielded a final codebook, which was used to re-code all responses.
% % % Any remaining disagreements were reconciled by the two coders.
% % % We report the codes and their distribution in Appendix B, along
% % % with the answers to all closed-ended questions.

% %\pushkal{There are significant differences in reading age and normal scores across party pages. One thing to note that quality score from another section also has similar model which gives based on words, sections etc.}

% %\miriam{can you correlate reading score with age of voters?}
% %\pushkal{By Edward The best source of demographic data for elections is the British Election Study
% %\url{https://www.britishelectionstudy.com/data/\#.XkbD9mj7Tcs}}

% % % \subsection{Quality score}
% % % Completeness of sections~\cite{piccardi2018structuring} and wikidata ~\cite{ahmeti2017assessing}


% %%%%%%%%%%%%%


==> sections/quality.tex <==
% \section{Quality of Wikipedia}\label{sec:quality}
% %Taking the word count for each MP page we find that the mean is 1051, median is 736 and highest is 13k for MP and former Labour party leader \emph{Jeremy Corbyn}, showing that MP pages vary significantly in length.\pushkal{This section can be written as a fusion of dynamics and polarisation that relates to good quality pages. For example high viewed pages are good? Polarised groups edit better? etc.} 
% We now move to analyze the quality of MPs' Wikipedia pages. We start by analyzing the quality of content which editors add. We operationalize the notion of quality through existing measures of article quality, citation quality and text readability% to develop an overall measure of quality
% . First, we make use of the ORES Wikimedia API~\cite{ores} to obtain, for each article, a quality score, similar to~\cite{Redi:2019:CNT:3308558.3313618}. For citation quality, we check if a statement needs a citation and if it has a citation or not using the test developed by~\cite{Redi:2019:CNT:3308558.3313618}. Finally, we compute articles' readability using Flesch-Kincaid~\cite{si2001statistical} and other readability scores.
% We provide a detailed explanation of the models used and the quality analysis result in the following subsections.


% %Using a single figure star for all 3 quality plots
% \begin{figure*}[thb]
%     \centering
%     \subfloat[Citation Quality] {
%         \includegraphics[width=0.33\textwidth]{figures/missingCitationBar.png}
%         %\label{fig:citation}
%     }
%     \subfloat[Readability] {
%         \includegraphics[width=0.33\textwidth]{figures/readingPartyMain.png}
%         \label{fig:reading}
%     }
%     \subfloat[Article Quality] {
%         \includegraphics[width=0.33\textwidth]{figures/qualityPrediction.png}
%         \label{fig:quality}
%     }
%     \caption{Dimension of pages quality. (a) Percentage of sentences which miss citation. (b) Reading Grade (RG) of main and page content per party. (c) Prediction of quality category. Darker the shade better is the page quality.}
%     \vspace{-0.5cm}
% \end{figure*}
    
    
% \subsection{Categories and Section}
% %The most frequently seen section headings are in Figure~\ref{fig:sectionTop}. 
% There are in total 11.5k sections on the 650 MP pages, with an average of 4 sections per MP articles (up to 14 for more popular MPs). %We find a total of 392 unique section titles and on average (as well as median) there are 4 sections which can be up to 14 for more popular MPs. 
% To assist our analysis of article quality, we manually group the 392 unique section titles into 12 labels% in two iterations
% , avoiding overlaps in the content covered by different labels as far as possible. The label with the highest percentage of words in relation to overall article length is \emph{Political and Parliamentary career} (56\%) which includes section headings such as Parliamentary career, Member of Parliament, House of Commons etc. Next we have \emph{Early life and career} (18\%) which includes section headings such as History, Education, Background, Early Career, etc. Other major labels are Main section (10\%), Personal life (6\%), Political views (5\%) and the rest cover the remaining 5\%. 

% To explore potential content biases, we breakdown section statistics party. %To understand whether at section level, take MPs' party and gender and ask if contributions to sections vary in size across these two categories.
% We compute the number of words for each section label, and aggregate over all articles of MPs of specific party (for example, we take the average number of words in Main Section of Conservatives and compare with the Main section of labour MPs, etc). %\pushkal{Paragraph updated. Need to add text based on Edward's comment here. EW: paragraph updated, let me know if i've got it right!}.
% To check significant differences in word count we perform the ANOVA test
% %\footnote{\url{www.sthda.com/english/wiki/one-way-anova-test-in-r}}
% on the resulting label distributions. %ased on average number of words for each category for each label type (for example, taking the average number of words in Main Section of Con:female, Lab:Female MPs, etc). 
% We get significant differences across categories for each of the three main labels -- Political and Parliamentary career ($p<0.001$), Early Life and Career ($p<0.05$) and Main Section ($p<0.001$). The distribution between political career and early life is different for each of the three main parties. In particular Conservative MPs' pages have slightly more about political career and less about early life as compared to Labour MPs. 
% %For Conservative, female MPs' pages have more about political career and less about early life than male MPs, whereas for Labour MPs, the distribution is similar for both male and female MPs. %For Labour, female MPs have more about political career, but less about early life than male MPs.
% %\pushkal{Removing plot of categories and section stacked bar. This is covered in text.}

% % We see from Figure~\ref{fig:partyGenderReference} that for SNP MPs, the main section comprises a larger fraction of the page. This is indicative of the rest of the page containing less detailed information in other categories such as political views and (in the case of female SNP MPs) political career. %We next see female MPs from SNP and others have less proportion of Political and Parliamentary career. A possible reason could be that female MPs are represented more in the Parliament in recent year elections than previously and hence have less records\footnote{\url{en.wikipedia.org/wiki/Women_in_the_House_of_Commons_of_the_United_Kingdom}, Accessed on 16 March 2020}. \pushkal{We need to add more details from new figure now.} 

% % \begin{figure}
% % \centering
% % %\includegraphics[width=\columnwidth]{figures/sectionPartyWordsBar.png}
% % \includegraphics[width=\columnwidth]{figures/sectionPartyWordsBar12Cat.png}
% % \caption{Stacked Bar plot of words count in section for each party and gender pair.
% % }~\label{fig:partyGenderReference}
% % \vspace{-0.5cm}

% % \end{figure}



% \subsection{Readability}
% %One way of specialisation can be a writing style. 
% The next dimension of quality we analyze is readability of articles. We compute this as reading grade of the article's body, and its main section.
% %As expected, we find that the main section  is easier to read than the article's body. We find that median Flesh \miriam{How does this compare to the rest of the Wikipedia?}
% We use a method similar to ~\cite{brezar2019readability} to compute Reading Grade ($RG$) which is the near equivalent of reading age. This involves computing the average of 
% Flesch--Kincaid ($FK$),  Simple Measure of Gobbledygook ($SMOG$) and Gunning Frequency of Gobbledygook ($FOG$) scores.~\cite{si2001statistical,benoit2018quanteda} We compute these after removing links, punctuation (except `.' and `,') and references to citations using R package~\cite{benoit2018quanteda}. We formally define Reading Grade ($RG$) as follows:

% \begin{equation}
%  RG=\frac{FK+SMOG+FOG}{3}
% \end{equation}
% %\ns{is this your definition? If so, why is taking a mean of the three scores useful? And are they all on the same scale from 0-100? If not you cannot just merge them in a linear fashion. }\pushkal{We use this formula from~\cite{brezar2019readability} as stated above.}
% We plot $RG$ of main section and page content of each MP page in Figure~\ref{fig:reading}. We see that main sections (median $RG=15.55$) are easier to read than page content ($RG=18.15$). In~\cite{brezar2019readability}, the authors report that the average $RG$ of the twenty-five most-viewed Wikipedia pages on diseases is 12.73 (sd: 0.32). This shows that over the years disease pages become easy to read with high and significant correlation between $FK$, $SMOG$ and $FOG$. They categorise $RG$ scores as under 12--fairly difficult (High school), 12 to 14--difficult (College level) and above 14--very difficult (College graduate level). We check percentage of main section and page content of MP articles based on this categorisation. We find that the main section of 9\% of pages are fairly difficult, 21\% are difficult and 70\% are very difficult. For overall page content 0.6\% of pages are fairly difficult, 1\% are difficult and the rest 98\% are very difficult. %\pushkal{Are we interested in knowing what are these difficult sections of the page content? EW: It would be more interesting to know why the pages are so difficult, but that will have to wait for another paper!}

% We also break down the $RG$ score by party, and find that Labour and SNP pages are easier to read than Conservative (KS-stats: (Con, Lab) D=0.16 and p<0.001, (Con, SNP) D=0.34, p<0.001). We show per party distribution in Figure~\ref{fig:reading}.%\pushkal{These numbers are distance in the distribution and if that if significant or not.}


% \subsection{Article Quality}
% The ORES~\cite{ores} API computes the probability of an article belonging to a given quality category  based on page length, infobox, number of images, sections etc. Given an article, ORES returns 6 probability scores, one for each quality level (\textit{Start, Stub, C-level (C), B-level (B), Good Article (GA), Featured Article (FA)})\footnote{More info- \url{en.wikipedia.org/wiki/Wikipedia:Content_assessment\#Grades}}.

% In Figure~\ref{fig:quality} we show the average quality score for each quality category, broken down by MPs' parties. %(known as \emph{articlequality}) which we use from Wikimedia API  which is a \emph{drafttopic} classifier~\cite{  asthana2018few,Redi:2019:CNT:3308558.3313618}. Similar to~\cite{halfaker2017interpolating, Redi:2019:CNT:3308558.3313618} we use ORES's \emph{articlequality} model which predict level of quality of an article
% %In Figure~\ref{fig:quality} we shows the predicted category based on eight quality categories provided by ORES. 
% Darker shades correspond to better page quality labels.
% We observe two major trends. First, despite the high overall citation quality, the quality of articles is largely poor: the majority of the articles for all parties are marked as ``C-level'', namely articles which are substantial but are  ``still missing important content or may still have significant problems which require substantial cleanup''.
% Second, we observe that articles on Conservative MPs tend to be of overall higher quality. To test if this is statistically significant %Additionally 
% we perform the ANOVA test, by converting quality category labels to numerical values such that 0 is Stub and 5 is Feature Article.  We find that there is a significant difference ($p<0.001$) in the ratings of articles across parties.

    
% % \begin{figure}
% % \centering
% % \includegraphics[width=0.8\columnwidth]{figures/qualityPrediction.png}
% %   \caption{Prediction of quality category of page. Darker the shade better is the page quality. }~\label{fig:quality}
% %   \vspace{-0.5cm}
% % \end{figure}
% % \begin{figure}
% % \centering
% %   \includegraphics[width=0.9\columnwidth]{figures/missingCitationBar.png}
% %   \caption{Percentage of sentences which miss citation according to citation needed scores.}~\label{fig:citation}
% %   \vspace{-0.5cm}
% % \end{figure}
% % \begin{figure}
% % \centering
% % %  \includegraphics[width=0.9\columnwidth]{figures/readingScore.png}
% %   \includegraphics[width=0.9\columnwidth]{figures/readingPartyMain.png}
% %  % \includegraphics[width=0.9\columnwidth]{figures/readingPartyMainFS.png}
% %   \caption{Reading Grade (RG) of main and page content per party. }~\label{fig:reading}
% %   \vspace{-0.5cm}
% % \end{figure}





% % UK population as per
% % \url{https://www.ons.gov.uk/peoplepopulationandcommunity/populationandmigration/populationestimates/articles/overviewoftheukpopulation/february2016} in 2014 Population aged
% % 0 to 15 (18.8\%), Population aged
% % 16 to 64 (63.5\%), Population aged 65
% % and over (17.7\%).

% % % https://www.syssec.ruhr-uni-bochum.de/media/emma/veroeffentlichungen/2019/09/05/uninformed-consent\_Yl7FPEh.pdf
% % % Emergent thematic coding

% % % Two of the authors independently devised a set of codes for each
% % % question and coded the responses. The results were discussed and
% % % yielded a final codebook, which was used to re-code all responses.
% % % Any remaining disagreements were reconciled by the two coders.
% % % We report the codes and their distribution in Appendix B, along
% % % with the answers to all closed-ended questions.

% %\pushkal{There are significant differences in reading age and normal scores across party pages. One thing to note that quality score from another section also has similar model which gives based on words, sections etc.}

% %\miriam{can you correlate reading score with age of voters?}
% %\pushkal{By Edward The best source of demographic data for elections is the British Election Study
% %\url{https://www.britishelectionstudy.com/data/\#.XkbD9mj7Tcs}}

% % % \subsection{Quality score}
% % % Completeness of sections~\cite{piccardi2018structuring} and wikidata ~\cite{ahmeti2017assessing}


% %%%%%%%%%%%%%

